Learning Symbolic Representations for Reinforcement Learning of Non-Markovian Behavior

Many real-world reinforcement learning (RL) problems necessitate learning complex, temporally extended behavior that may only receive reward signal when the behavior is completed. If the reward-worthy behavior is known, it can be specified in terms of a non-Markovian reward function - a function that depends on aspects of the state-action history, rather than just the current state and action. Such reward functions yield sparse rewards, necessitating an inordinate number of experiences to find a policy that captures the reward-worthy pattern of behavior. Recent work has leveraged Knowledge Representation (KR) to provide a symbolic abstraction of aspects of the state that summarize reward-relevant properties of the state-action history and support learning a Markovian decomposition of the problem in terms of an automaton over the KR. Providing such a decomposition has been shown to vastly improve learning rates, especially when coupled with algorithms that exploit automaton structure. Nevertheless, such techniques rely on a priori knowledge of the KR. In this work, we explore how to automatically discover useful state abstractions that support learning automata over the state-action history. The result is an end-to-end algorithm that can learn optimal policies with significantly fewer environment samples than state-of-the-art RL on simple non-Markovian domains.

==> coverpage.tex <==
\newcommand{\alternate}[1]{\textcolor{blue}{#1}}
\newcommand{\changes}[1]{\textcolor{red}{#1}}
\newcommand{\remove}[1]{\textcolor{green}{#1}}
\newcommand{\shorten}[1]{\textcolor{orange}{#1}}
\newcommand{\todiscuss}[1]{\textcolor{brown}{#1}}
\newcommand{\commentsm}[1]{\textcolor{cyan}{{\bf SM: }#1}}
\newcommand{\commentpc}[1]{\textcolor{cyan}{{\bf PC: }#1}}
\newcommand{\commental}[1]{\textcolor{cyan}{{\bf AL: }#1}}
\newcommand{\commentrt}[1]{\textcolor{cyan}{{\bf RT: }#1}}

\section*{Colour Legend}

\textcolor{red}{Red text highlights changes to note (uses "$\backslash$changes")}\\
\textcolor{blue}{Blue text suggests an alternative phrasing to the one in the preceding sentence or paragraph (uses "$\backslash$alternate")}\\
\textcolor{green}{Green text is marked for potential removal, mostly to shorten the document (uses "$\backslash$remove")}\\
\textcolor{brown}{Brown text is marked for discussion (uses "$\backslash$remove")}\\
\textcolor{orange}{Orange text marks a body of text that is very nice but that I am suggesting be shortened, again mostly to shorten the overall document (uses "$\backslash$shorten")}\\
\textcolor{cyan}{Cyan text, preceded by "SM: " is inserted comments. (uses "$\backslash$commentsm")\\
Similarly for everyone else, i.e., "$\backslash$commentpc", "$\backslash$commental", "$\backslash$commentrt"}





\section*{General things to watch for}
\begin{itemize}
    \item inconsistent spelling: ({\bf behavior}, behaviour)
\end{itemize}

\newpage




==> macroadmin.tex <==

\newif\ifcomments
% Set the following variable to change between clean version and commented one.
\commentstrue
% \commentsfalse

% \newcommand{\plagia}[1]{\textcolor{red}{\sout{#1}}}
\ifcomments
%%%%%%%%%%%%%%%%%%%


\newcommand{\debate}[1]{\textcolor{green}{#1}}
\newcommand{\debating}[1]{\textcolor{black}{#1}}
\newcommand{\promised}[1]{\textcolor{red}{\bf **Promised in paper**: {#1}}}
\newcommand{\toresolve}[1]{\textcolor{yellow}{#1}}
\newcommand{\remove}[1]{\textcolor{green}{#1}}
\newcommand{\alt}[1]{\textcolor{brown}{#1}}
\newcommand{\commentsm}[1]{\textcolor{magenta}{({\bf SM:} #1)}}
\newcommand{\commentpc}[1]{\textcolor{red}{({\bf PC:} #1)}}
\newcommand{\commental}[1]{\textcolor{cyan}{({\bf AL:} #1)}}
\newcommand{\commentrti}[1]{\textcolor{green}{({\bf rti:} #1)}}
\newcommand{\old}[1]{\textcolor{red}{\sout{#1}}}
\newcommand{\new}[1]{\textcolor{BrickRed}{\uline{#1}}}
\else
%%%%%%%%%COMMENTS NOT VISIBLE%%%
 \newcommand{\old}[1]{}
 \newcommand{\new}[1]{#1}
%%%%%%%%%%%%%%%%%%%%%%%
\fi


% "revisit" is intended for things we need to check later. It can be used, for example to highlight things we're not sure we really ended up doing (so may wish to remove or de-emphasize).
\newcommand{\revisit}[1]{\textcolor{black}{#1}}
